UniT3D: A Unified Transformer for 3D Dense Captioning and Visual Grounding

Performing 3D dense captioning and visual grounding requires a common and shared understanding of the underlying multimodal relationships. However, despite some previous attempts on connecting these two related tasks with highly task-specific neural modules, it remains understudied how to explicitly depict their shared nature to learn them simultaneously. In this work, we propose UniT3D, a simple yet effective fully unified transformer-based architecture for jointly solving 3D visual grounding and dense captioning. UniT3D enables learning a strong multimodal representation across the two tasks through a supervised joint pre-training scheme with bidirectional and seq-to-seq objectives. With a generic architecture design, UniT3D allows expanding the pre-training scope to more various training sources such as the synthesized data from 2D prior knowledge to benefit 3D vision-language tasks. Extensive experiments and analysis demonstrate that UniT3D obtains significant gains for 3D dense captioning and visual grounding.

==> figures/overview.tex <==
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.99\linewidth]{assets/overview.pdf}
    \vspace{-3mm}
    \caption{We propose~\ARCH, a transformer architecture for unified 3D vision-language pre-training.~\ARCH~is pre-trained with both bidirectional and seq-to-seq objectives on point-cloud-text pairs. After the pre-training stage,~\ARCH~is further fine-tuned separately for 3D visual grounding and dense captioning with lightweight task-specific heads. We show that the pre-trained knowledge clearly improves the overall accuracy on both downstream tasks. \Xinlei{(minor) "Unified Transformer" is abbreviated for the captioning task, and there is ... in between -- is it indicating more than 2 tasks?}}
    \label{fig:overview}
    \vspace{-6mm}
\end{figure}
